Attributed Hierarchical Port Graphs and Applications

We present attributed hierarchical port graphs (AHP) as an extension of port graphs that aims at facilitating the design of modular port graph models for complex systems. AHP consist of a number of interconnected layers, where each layer defines a port graph whose nodes may link to layers further down the hierarchy; attributes are used to store user-defined data as well as visualisation and run-time system parameters. We also generalise the notion of strategic port graph rewriting (a particular kind of graph transformation system, where port graph rewriting rules are controlled by user-defined strategies) to deal with AHP following the Single Push-out approach. We outline examples of application in two areas: functional programming and financial modelling.

==> eptcsdata.tex <==
\providecommand{\firstpage}{2}
\providecommand{\publicationstatus}{H. Cirstea, D. Sabel (Eds.): Fourth International Workshop on Rewriting\\
Techniques for Program Transformations and Evaluation (WPTE 2017)\\
EPTCS 265, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.265.2}{10.4204/EPTCS.265.2}}
\pdfoutput=1

